Causal Attention for Vision-Language Tasks

We present a novel attention mechanism: Causal Attention (CATT), to remove the ever-elusive confounding effect in existing attention-based vision-language models. This effect causes harmful bias that misleads the attention module to focus on the spurious correlations in training data, damaging the model generalization. As the confounder is unobserved in general, we use the front-door adjustment to realize the causal intervention, which does not require any knowledge on the confounder. Specifically, CATT is implemented as a combination of 1) In-Sample Attention (IS-ATT) and 2) Cross-Sample Attention (CS-ATT), where the latter forcibly brings other samples into every IS-ATT, mimicking the causal intervention. CATT abides by the Q-K-V convention and hence can replace any attention module such as top-down attention and self-attention in Transformers. CATT improves various popular attention-based vision-language models by considerable margins. In particular, we show that CATT has great potential in large-scale pre-training, e.g., it can promote the lighter LXMERT~\cite{tan2019lxmert}, which uses fewer data and less computational power, comparable to the heavier UNITER~\cite{chen2020uniter}. Code is published in \url{https://github.com/yangxuntu/catt}.

==> temp_approach.tex <==
\section{Causal Attention}
\subsection{Attention vs. Front-Door Principle}
%简单描述一下attention based model的过程：attention mechanism选区域，predictor来预测, chain together a selector and a predictor
We retrospect attention mechanism by comparing it with the front-door principle, which is used to estimate the causal effect of the current input $\mathcal{X}$ on the target $\mathcal{Y}$ when the confounder is not observable~\cite{PearlMackenzie18,pearl2000causality}. Formally, attention mechanism calculates the observational correlation as:
% \begin{equation} \label{equ:attention}
% % \begin{aligned}
%   &P(\mathcal{Y}|\mathcal{X}) \\ &=\underbrace{\sum\nolimits_{\bm{z}}P(\bm{z}|\mathcal{X})}_{\text{In-Sample}}{P(\mathcal{Y}|\bm{z})} %\\
%     %&= \mathbb{E}_{[\bm{z}|\mathcal{X}]}[P(\mathcal{Y}|\bm{z})],
%     % \end{aligned}
% \end{equation}
\begin{equation} \label{equ:attention}
   P(\mathcal{Y}|\mathcal{X})  =\underbrace{\sum\nolimits_{\bm{z}}P(\bm{z}|\mathcal{X})}_{\text{IS-EXPT}}{P(\mathcal{Y}|\bm{z})} 
\end{equation}
and the front-door principle estimates the causal effect as:
\begin{equation} \label{equ:front_door}
\begin{aligned}
    &P(\mathcal{Y}|do(\mathcal{X})) \\
    = &\underbrace{\sum\nolimits_{\bm{z}}P(\bm{z}|\mathcal{X})}_{\text{IS-EXPT}}\underbrace{\sum\nolimits_{\bm{x}}P(\bm{x})}_{\text{CS-EXPT }}[P(\mathcal{Y}|\bm{x},\bm{z})] 
    %\\= &\mathbb{E}_{[\bm{z}|\mathcal{X}]}[\mathbb{E}_{\mathcal{X}'}[P(\mathcal{Y}|\mathcal{X}',\bm{z})]],
\end{aligned}
\end{equation}
where $\bm{z}$, $\bm{x}$ denote the value from the current sample and all the other possible samples and $do(\cdot)$ denotes the interventional operation~\cite{PearlMackenzie18,pearl2000causality}. The key difference between them is that $P(\mathcal{Y}|do(\mathcal{X}))$ not only calculates the expectation in the current sample $\mathcal{X}$: $\mathbb{E}_{[\bm{z}|\mathcal{X}]}[\cdot]$, hence denoted as In-Sample Expectation (\textbf{IS-EXPT}), but also marginalizes over all the other potential samples $\bm{x}$: $\mathbb{E}_{\bm{x}}[\cdot]$, hence denoted as Cross-Sample Expectation (\textbf{CS-EXPT}).
% \begin{equation} \label{equ:attention_network}
% \begin{aligned}
%  \textbf{IS-EXPT:} \quad  & \mathbb{E}_{[\bm{z}|\mathcal{X}]}[f(\bm{z})] =  \sum\nolimits_{\bm{z}}P(\bm{z}|\mathcal{X})[f(\bm{z})]\\
%  \textbf{CS-EXPT:} \quad  & \mathbb{E}_{\mathcal{X}'}[f(\mathcal{X}')] = \sum\nolimits_{\mathcal{X}'}P(\mathcal{X}')[f(\mathcal{X}')]\\
% \end{aligned}
% \end{equation}
% \begin{equation} \label{equ:attention_network}
% \begin{aligned}
%  \textbf{IS-EXPT:} \quad  & \mathbb{E}_{[\bm{z}|\mathcal{X}]}[\cdot], \\
%  \textbf{CS-EXPT:} \quad  & \mathbb{E}_{\mathcal{X}'}[\cdot].
% \end{aligned}
% \end{equation}

Attention mechanism (Eq.~\eqref{equ:attention}) calculates the predictive distribution $P(\mathcal{Y}|\bm{z})$ for each selected $\bm{z}$ during IS-EXPT. However, since attention mechanism is an unsupervised process, it does not know which selected $\bm{z}$ is correct or not for predicting the current target and then the predictor may be disturbed by the spurious correlation brought by the dataset bias. For example, given an image with ``man-with-skateboard'', the predictor does not know whether the person region or skateboard region is the suitable evidence for predicting the word ``man''. However, since most images containing a skateboard are annotated by ``man-with-skateboard''~\cite{hendricks2018women}, the predictor has the chance to incorrectly treat the skateboard region as the evidence for predicting ``man''. In this way, attention mechanism learns to build the spurious correlation between the skateboard region with the word ``man. As a result, during test, given an image containing ``woman-with-skateboard'', such a model may directly predict the gender as ``man'' after observing the skateboard region.

However, in the front-door principle (Eq.~\eqref{equ:front_door}), CS-EXPT approximates the ``physically intervention'' by combining a selected region, \eg, the person region, with all the other objects, \eg, skateboard, mirror, or brush, to break the strong correlation between ``man-with-skateboard'' caused by the hidden confounder. Then the predictor will infer the word ``man'' only when the person region is given, which thus forces the attention mechanism to focus on the suitable region, \ie, having a high probability $P(\bm{z}|\mathcal{X})$ when $\bm{z}$ is about the person. To sum up, we can see that CS-EXPT corrects the predictor $P(\mathcal{Y}|\bm{x},\bm{z})$ from the dataset bias and then further instructs attention mechanism to select the suitable region. In this way, if we follow the front-door principle (Eq.~\eqref{equ:front_door}) to design a model, it will be more robust than the traditional attention network which is designed based on Eq.~\eqref{equ:attention}. Since $P(\mathcal{Y}|do(\mathcal{X}))$ estimates the causal effect of $\mathcal{X}$ on $\mathcal{Y}$, we name our model as causal attention (CATT). 


\subsection{In-Sample and Cross-Sample Attentions}
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 5mm 5mm 5mm,clip]{latex/fig_arch.pdf}
   \caption{ 
   }
\label{fig:arch}
\end{figure}

From Eq.~\eqref{equ:front_door}, we can see that the crux of causal attention is the implementation of IS-EXPT and CS-EXPT, while the attention network has implemented the former one by proposing the Q-K-V operation. Similarly, it can also be exploited to estimate the CS-EXPT value. To distinguish them, we name the former and latter networks as In-Sample attention (IS-ATT) and Cross-Sample attention (CS-ATT). When applying our causal attention in the other architectures, we set IS-ATT to the same as the original attention network to estimate IS-EXPT. For CS-ATT, we apply the multi-head scaled dot-product operation~\cite{vaswani2017attention} to estimate CS-EXPT. Formally, given the query, key, and value sets $\bm{Q}$, $\bm{K}$, and $\bm{V}$, the output representation set $\hat{\bm{V}}$ is calculated as:
\begin{equation} \label{equ:multi-head}
\small
\begin{aligned}
 \textbf{Input:} \quad  &\bm{Q},\bm{K},\bm{V} \\
 \textbf{Prob:} \quad  &\bm{A}_i=\text{Softmax}( \frac{\bm{Q}\bm{W}_i^Q(\bm{K}\bm{W}_i^K)^T}{\sqrt{d}} ) \\
 \textbf{Single-Head}:  \quad  &\bm{H}_i=\bm{A}_i\bm{V}\bm{W}_i^V,\\
 \textbf{Ouput:} \quad & \hat{\bm{V}}= [\bm{H}_1,\bm{H}_2,...,\bm{H}_h]\bm{W}^H,
\end{aligned}
\end{equation}
where $\bm{W}_i^Q, \bm{W}_i^K, \bm{W}_i^V$, and $\bm{W}_i^H$ are all trainable matrices; $h$ is the number of the heads; $\bm{A}_i$ is the attention matrix for calculating the $i$-th head matrix $\bm{H}_i$; and $[\cdot]$ denotes the concatenation operation. Compared with IS-ATT which usually specifies $\bm{Q}$, $\bm{K}$, and $\bm{V}$ as the representation set of the current sample, \eg, the RoI representations of the objects in an image, in CS-ATT, we set $\bm{K}$ and $\bm{V}$ to the global dictionary compressed from the whole training set, \eg, initializing them by applying K-means algorithm over the RoI representations of all the training images. To increase the flexibility of CS-ATT, the query $\bm{Q}$ can be specified as different representation sets case by case.

\subsection{CATT in Various Architectures}
In the experiments, we implement our causal attention into three different encoder-decoders: Bottom-Up Top-Down (BUTD) LSTM~\cite{anderson2018bottom}, Transformer~\cite{vaswani2017attention}, and a large scale vision-language pre-training framework LXMERT~\cite{tan2019lxmert}. Here we detail how to use our causal attention to replace various attention modules in these architectures.



%where the Q-K-V operations of IS-ATT and CS-ATT are specified by different formations. Generally, we implement our IS-ATT as the original attention networks in these architectures and change the settings of CS-ATT case by case. We detail the applied settings based on the sketched architecture in Fig.~\ref{fig:arch} and the Q-K-V operation defined in Eq.~\eqref{equ:attention_network} as follows.

% \noindent\textbf{BUTD.} Only the guided-attention is used here, which is called the Bottom-Up attention model~\cite{anderson2018bottom} and we set this guided-attention as our IS-ATT.  $\bm{V}$, $\bm{K}$ are both set to the RoI representations of the objects in an image and the query $\bm{q}$ is the embedding of the sentence context, \eg, the partially generated caption and the question for image captioning and VQA, respectively. The mapping function $f(\cdot)$ is:
% \begin{equation} \label{equ:sum_attention}
%     f(\bm{k},\bm{q}) = \bm{w}^T(\bm{W}_k\bm{k}+\bm{W}_q\bm{q}),
% \end{equation}
% where $\bm{w}$ is a trainable vector and $\bm{W}_k$, $\bm{W}_q$ are two trainable matrices. 

% For CS-ATT, we set the query as the same one in IS-ATT, and $\mathcal{V}$, $\mathcal{K}$ are set to the same visual global dictionary $\bm{X}$, which is initialized by applying K-means over all the RoI features in the training dataset, where $K$ is set to 5000. Considering dot product is more efficient than the sum operation in Eq.~\eqref{equ:sum_attention} and the value set is much bigger than the one in IS-ATT, we apply the one-head scaled dot-product attention:
% \begin{equation} \label{equ:dot_attention}
%     f(\bm{k},\bm{q}) = \bm{k}^T\bm{q}/\sqrt{d_k},
% \end{equation}
% where $d_k$ is the dimension of the vector $\bm{k}$.

% After calculating $\hat{\bm{z}}$ and $\hat{\bm{x}}$ from IS-ATT and CS-ATT, respectively, they are concatenated and then input into the last few layers for calculating the predictive distributions.

% \noindent\textbf{Transformer.} It is built by stacking a few self-attention and top-down attention layers and all of these layers apply multi-head scaled dot-product to calculate the attended values with different inputs.


% which is called multi-head scaled dot-product operation:

% Both the self-attention and guided-attention are used here and we replace all of them with our CATT. All of the IS-ATT and CS-ATT in self-attention and guided-attention have the same Q-K-V operations with different inputs. Specifically, they apply multi-head scaled dot-product operation:
% \begin{equation} \label{equ:multi-head}
% \small
% \begin{aligned}
%  \textbf{Input:} \quad  &\bm{Q},\bm{K},\bm{V} \\
%  \textbf{Att:} \quad  &\bm{A}_i=\text{Softmax}( \frac{\bm{Q}\bm{W}_i^Q(\bm{K}\bm{W}_i^K)^T}{\sqrt{d}} ) \\
%  \textbf{Head}:  \quad  &\bm{H}_i=\bm{A}_i\bm{V}\bm{W}_i^V,\\
%  \textbf{Multi-Head:} \quad & \bm{H}= [\bm{H}_1,\bm{H}_2,...,\bm{H}_8]\bm{W}^H,
% \end{aligned}
% \end{equation}
% In self-attention, for IS-ATT, $\bm{Q}=\bm{K}=\bm{V}=\bm{Z}$ and for CS-ATT, $\mathcal{K}=\mathcal{V}=\bm{X}$ and $\mathcal{Q}=\bm{Z}$, where $\bm{Z}$ can be the RoI representations of an image or the word embeddings of a sentence and $\bm{X}$ is the corresponding global dictionary initialized by applying K-means over the RoI representations or word embeddings of the whole training dataset. 




% By comparing Eq.~\eqref{equ:front_door} with~\eqref{equ:attention}, we can see the key difference is that $P(\mathcal{Y}|do(\mathcal{X}))$ not only calculates the expectation in the current sample $\mathcal{X}$, but also marginalizes over all the other potential samples $\bm{x}$, hence denoted as Cross-Sample Expectation (\textbf{CS-EXPT}). Actually, CS-EXPT approximates the ``physically intervention'' by combining a selected region, \eg, the person region, with all the other objects, \eg, skateboard, mirror, or brush, to break the strong correlation between ``man-with-skateboard'' caused by the hidden confounder. Then the predictor will infer the word ``man'' only when the person region is given, which thus forces the attention mechanism to focus on the suitable region, \ie, having a high probability $P(\bm{z}|\mathcal{X})$ when $\bm{z}$ is about the person. To sum up, we can see that CS-EXPT corrects the predictor $P(\mathcal{Y}|\bm{x},\bm{z})$ from the dataset bias and then further instructs attention mechanism to select the suitable region. In this way, if we follow the front-door principle (Eq.~\eqref{equ:front_door}) to design a model, it will be more robust than the traditional attention network which is designed based on Eq.~\eqref{equ:attention}. Since $P(\mathcal{Y}|do(\mathcal{X}))$ estimates the causal effect of $\mathcal{X}$ on $\mathcal{Y}$, we name our model as causal attention (CATT). 


% \begin{equation} \label{equ:front_door}
% \begin{aligned}
%     &P(\mathcal{Y}|do(\mathcal{X})) \\
%     = &\underbrace{\sum\nolimits_{\bm{z}}P(\bm{z}|\mathcal{X})}_{\text{IS-EXPT}}\underbrace{\sum\nolimits_{\bm{x}}P(\bm{x})}_{\text{CS-EXPT }}[P(\mathcal{Y}|\bm{x},\bm{z})] 
% \end{aligned}
% \end{equation}
% where $\bm{z}$, $\bm{x}$ denote the value from the current sample and all the other possible samples and $do(\cdot)$ denotes the interventional operation~\cite{PearlMackenzie18,pearl2000causality}. The key difference between them is that $P(\mathcal{Y}|do(\mathcal{X}))$ not only calculates the expectation in the current sample $\mathcal{X}$: $\mathbb{E}_{[\bm{z}|\mathcal{X}]}[\cdot]$, hence denoted as In-Sample Expectation (\textbf{IS-EXPT}), but also marginalizes over all the other potential samples $\bm{x}$: $\mathbb{E}_{\bm{x}}[\cdot]$, hence denoted as Cross-Sample Expectation (\textbf{CS-EXPT}).

% Attention mechanism (Eq.~\eqref{equ:attention}) calculates the predictive distribution $P(\mathcal{Y}|\bm{z})$ for each selected $\bm{z}$ during IS-EXPT. However, since attention mechanism is an unsupervised process, it does not know which selected $\bm{z}$ is correct or not for predicting the current target and then the predictor may be disturbed by the spurious correlation brought by the dataset bias. For example, given an image with ``man-with-skateboard'', the predictor does not know whether the person region or skateboard region is the suitable evidence for predicting the word ``man''. However, since most images containing a skateboard are annotated by ``man-with-skateboard''~\cite{hendricks2018women}, the predictor has the chance to incorrectly treat the skateboard region as the evidence for predicting ``man''. In this way, attention mechanism learns to build the spurious correlation between the skateboard region with the word ``man. As a result, during test, given an image containing ``woman-with-skateboard'', such a model may directly predict the gender as ``man'' after observing the skateboard region.

% However, in the front-door principle (Eq.~\eqref{equ:front_door}), CS-EXPT approximates the ``physically intervention'' by combining a selected region, \eg, the person region, with all the other objects, \eg, skateboard, mirror, or brush, to break the strong correlation between ``man-with-skateboard'' caused by the hidden confounder. Then the predictor will infer the word ``man'' only when the person region is given, which thus forces the attention mechanism to focus on the suitable region, \ie, having a high probability $P(\bm{z}|\mathcal{X})$ when $\bm{z}$ is about the person. To sum up, we can see that CS-EXPT corrects the predictor $P(\mathcal{Y}|\bm{x},\bm{z})$ from the dataset bias and then further instructs attention mechanism to select the suitable region. In this way, if we follow the front-door principle (Eq.~\eqref{equ:front_door}) to design a model, it will be more robust than the traditional attention network which is designed based on Eq.~\eqref{equ:attention}. Since $P(\mathcal{Y}|do(\mathcal{X}))$ estimates the causal effect of $\mathcal{X}$ on $\mathcal{Y}$, we name our model as causal attention (CATT). 















From Eq.~\eqref{equ:front_door}, we can see that the crux of causal attention is the implementation of IS-Sampling and CS-Sampling. Researchers propose Normalized Weighted Geometric Meaning approximation (NWGM)~\cite{xu2015show} to absorb IS-Sampling (Eq.~\eqref{equ:attention}) into the network:
\begin{equation}\label{equ:nwgm_isatt}
\begin{aligned}
    P(\mathcal{Y}|\mathcal{X})&=\sum\nolimits_{\bm{z}}P(\bm{z}|\mathcal{X})P(\mathcal{Y}|\bm{z})\approx \\
    &\text{Softmax}(\hat{\bm{z}}),\\
    \hat{\bm{z}} &= \sum\nolimits_{i}\alpha_i\bm{z}_i
\end{aligned}
\end{equation}




where $P(\mathcal{Y}|\bm{z})$ is parameterized by a network whose last layer is a Softmax layer and $\hat{\bm{z}}$ is what a conventional attention network calculates. Specifically, the calculation process is usually summarized as the Q-K-V operation as shown in Figure~\ref{fig:arch} (a), where $f(\cdot)$ encodes $\mathcal{X}$ and $\bm{z}$ to the value $\bm{V}$ and $P_{\alpha}$ denotes the calculated soft attention weights from the query $\bm{Q}$ and key $\bm{K}$. 

Similarly, we also exploit NWGM to implement Eq.~\eqref{equ:front_door}:
\begin{equation}\label{equ:nwgm_catt}
\begin{aligned}
    &P(\mathcal{Y}|do(\mathcal{X}))\approx \text{Softmax}(\hat{\bm{z}},\hat{\bm{x}}),\\
    &\hat{\bm{z}} = \sum\nolimits_{\bm{z}}f(\bm{z},\mathcal{X})P_{\alpha}(\bm{z}|\mathcal{X}),\\
    &\hat{\bm{x}} = \sum\nolimits_{\bm{x}}g(\bm{x})P_{\beta}(\bm{x}),\\
\end{aligned}
\end{equation}
where $\hat{\bm{z}}$ can be got by the conventional attention network as mentioned above.

% Similarly, we also exploit NWGM to implement CS-Sampling by the Q-K-V operation.
% To distinguish them, we name the former and latter modules as In-Sample attention (IS-ATT) and Cross-Sample attention (CS-ATT). When applying our causal attention modules in the other architectures, we set IS-ATT to the same as the original attention module. For CS-ATT, we implement it by the multi-head scaled dot-product~\cite{vaswani2017attention}. Formally, given the query, key, and value sets $\bm{Q}$, $\bm{K}$, and $\bm{V}$, the output representation set $\hat{\bm{V}}$ is calculated as:
% \begin{equation} \label{equ:multi-head}
% \small
% \begin{aligned}
%  \textbf{Input:} \quad  &\bm{Q},\bm{K},\bm{V} \\
%  \textbf{Prob:} \quad  &\bm{A}_i=\text{Softmax}( \frac{\bm{Q}\bm{W}_i^Q(\bm{K}\bm{W}_i^K)^T}{\sqrt{d}} ) \\
%  \textbf{Single-Head}:  \quad  &\bm{H}_i=\bm{A}_i\bm{V}\bm{W}_i^V,\\
%  \textbf{Ouput:} \quad & \hat{\bm{V}}= [\bm{H}_1,\bm{H}_2,...,\bm{H}_h]\bm{W}^H,
% \end{aligned}
% \end{equation}
% where $\bm{W}_i^Q, \bm{W}_i^K, \bm{W}_i^V$, and $\bm{W}_i^H$ are all trainable matrices; $h$ is the number of the heads; $\bm{A}_i$ is the soft attention weights matrix for calculating the $i$-th head matrix $\bm{H}_i$; and $[\cdot]$ denotes the concatenation operation. The output $\hat{\bm{V}}$ can be used to calculate the predictive distribution or be further embedded by more attention layers in different architectures.

% Compared with IS-ATT which usually specifies $\bm{Q}$, $\bm{K}$, and $\bm{V}$ as the representation sets of the current sample, \eg, the RoI representations of the objects in an image, in CS-ATT, we set $\bm{K}$ and $\bm{V}$ to the global dictionary compressed from the whole training set, \eg, initializing them by applying K-means algorithm over the RoI representations of all the training images. To increase the flexibility of CS-ATT, the query $\bm{Q}$ can be specified as different representation sets case by case. 

